Improving Conversational Recommender System via Contextual and Time-Aware Modeling with Less Domain-Specific Knowledge

Conversational Recommender Systems (CRS) has become an emerging research topic seeking to perform recommendations through interactive conversations, which generally consist of generation and recommendation modules. Prior work on CRS tends to incorporate more external and domain-specific knowledge like item reviews to enhance performance. Despite the fact that the collection and annotation of the external domain-specific information needs much human effort and degenerates the generalizability, too much extra knowledge introduces more difficulty to balance among them. Therefore, we propose to fully discover and extract internal knowledge from the context. We capture both entity-level and contextual-level representations to jointly model user preferences for the recommendation, where a time-aware attention is designed to emphasize the recently appeared items in entity-level representations. We further use the pre-trained BART to initialize the generation module to alleviate the data scarcity and enhance the context modeling. In addition to conducting experiments on a popular dataset (ReDial), we also include a multi-domain dataset (OpenDialKG) to show the effectiveness of our model. Experiments on both datasets show that our model achieves better performance on most evaluation metrics with less external knowledge and generalizes well to other domains. Additional analyses on the recommendation and generation tasks demonstrate the effectiveness of our model in different scenarios.

==> figures/limitation_dist_n.tex <==
\begin{figure}[t]
\caption{\label{fig:limit_distn} Change of Dist-2 and BLEU2 scores when using different length penalty. Larger length penalty ($>1$) indicates allowing generating longer responses.}
\centering
\includegraphics[width=0.45\textwidth]{mypictures/exp_dictn.pdf}
% \vskip -0.5em

% \vskip -0.5em
\end{figure}

==> figures/time_recency_lamda.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{mypictures/exp_rec_lamda_fig.pdf}
% \vskip -0.5em
\caption{\label{fig:rec_lamda} Change of Recall scores when using different values of $\lambda$, which controls the recency effect.}
\end{figure}

==> sections/abstract.tex <==
\begin{abstract}
Conversational Recommender Systems has become an emerging research topic seeking to perform recommendations through interactive conversations, which generally consist of generation and recommendation modules. Prior work on CRS tends to incorporate more external and domain-specific knowledge like item reviews to enhance performance. Despite the fact that the collection and annotation of the \textbf{external domain-specific} information need much human effort and degenerates the generalizability, too much extra knowledge introduces more difficulty to balance among them. Therefore, we propose to fully discover and extract the \textbf{internal} knowledge from the context. We capture both entity-level and contextual-level representations to jointly model user preferences for the recommendation, where time-aware attention is designed to emphasize the recently appeared items in entity-level representations. We further use the pre-trained BART to initialize the generation module to alleviate the data scarcity and enhance the context modeling. In addition to conducting experiments on a popular dataset (ReDial), we also include a multi-domain dataset (OpenDialKG) to show the effectiveness of our model. Experiments on both datasets show that our model achieves better performance on most evaluation metrics with less external knowledge and generalizes well to other domains. Additional analyses on the recommendation and generation tasks demonstrate the effectiveness of our model in different scenarios.
\end{abstract}

==> tables/algorithm.tex <==
\begin{algorithm}[t]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Vocabulary Pointer based Generation for RecInDial}\label{alg:cap}
\begin{algorithmic}
\Require history context $C$, general and item vocabulary $V_G$, $V_R$
\Ensure generated response $R$
\State extract appeared entities from $C$ as user preference $\mathcal{T}_u$
\State compute knowledge-aware bias $\bm{b}_u$ based on $\mathcal{T}_u$ using Eq.~\ref{eq:entity} to \ref{eq:bias}
\State $R \gets \{\}$
\State $n \gets 0$
\State $I_{vp} \gets 0$, $V \gets V_G$
\While{$n < N_{max}$} 
\State \textcolor[rgb]{0.6,0.6,0.6}{\# Generate $w_n$ based on the previous tokens and bias from $V$}
\State $w_n = Decode(C \bigcup R, V, \bm{b}_u)$
\State $R \gets R \bigcup\{w_n\}$
\If{$w_n = [RecS]$} \textcolor[rgb]{0.6,0.6,0.6}{\Comment{Start to generate tokens from $V_R$}}
\State $I_{vp} \gets 1$, $V \gets V_R$
\ElsIf{$w_n = [RecE]$}
\textcolor[rgb]{0.6,0.6,0.6}{\Comment{Start to generate tokens from $V_G$}}
\State $I_{vp} \gets 0$, $V \gets V_G$
\ElsIf{$w_n = [EOS]$}
\textcolor[rgb]{0.6,0.6,0.6}{\Comment{Generation is done}}
\State \textbf{break}
\EndIf
\State $n \gets n+1$
\EndWhile
\State \textbf{return} R
\end{algorithmic}
\end{algorithm}
